The Dynamic Creativity of Proto-artifacts in Generative Computational Co-creation

This paper explores the attributes necessary to determine the creative merit of intermediate artifacts produced during a computational co-creative process (CCC) in which a human and an artificial intelligence system collaborate in the generative phase of a creative project. In an active listening experiment, subjects with diverse musical training (N=43) judged unfinished pieces composed by the New Electronic Assistant (NEA). The results revealed that a two-attribute definition based on the value and novelty of an artifact (e.g., Corazza's effectiveness and novelty) suffices to assess unfinished work leading to innovative products, instead of Boden's classic three-attribute definition of creativity (value, novelty, and surprise). These findings reduce the creativity metrics needed in CCC processes and simplify the evaluation of the numerous unfinished artifacts generated by computational creative assistants.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sections/03_Ev_Computational_Co-Creativity.tex <==
%The CC community has developed several perspectives for evaluating creativity in ideas and artifacts produced by a system, most of them classifiable in the four P taxonomy: person, process, product, and press (the culture that influences and judges creative people, processes and products) \cite{rhodes1961analysis,jordanous2016four,lamb2018evaluating}. Given that CCC is a subfield of CC, one would expect that the second P (process:the actions taken to produce a creative piece) would encompass some guidelines for evaluating CCC process. But, the four P framework is more descriptive than evaluative \cite{lamb2018evaluating}.

%In traditional CC processes are commonly described as iterative structures 
%\cite{wallas1926art,sadler2015wallas,csikszentmihalyi1997flow,simonton2011creativity,ward_smith_finke_1998,amabile2011componential} and can be roughly characterized as recursive iterations over two primary sub-processes: producing artifacts and judging them. However, it is not clear how or what to measure in each sub-process, even less in the context of a human-artificial agent collaboration. Such indetermination has been a known challenge for CC evaluation frameworks such as FACE \cite{colton2011computational} and SPECS \cite{jordanous2012standardised} because subjects fail to understand the concepts used in the assessment or because the assessment relies on subjects’ knowledge of the inner workings of the systems being evaluated \cite{lamb2018evaluating}. Nowadays, the question of how to evaluate computational creativity remains open and continues to mature as technical and social applications of systems evolve. More so if CCC systems entail collaborative work in the arts and humanities \cite{yang2020evaluation}. The following section contributes to this discussion by proposing a conceptual framework to assess the co-creation process in the context of a partnership between a human and an AI system.















==> sections/07_Generation.tex <==



==> sections/14_results.tex <==
Three subjects with high musical training consistently scored the same control stimuli with a difference of more than 3 points for all three attributes (value, surprise, and novelty). Therefore, all their responses were discarded due to inconsistency.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{dist_scores}
    \caption{Distribution of novelty, surprise and value scores among all participants and all pieces}
    \label{fig:dist_scores}
\end{figure}

\textbf{Are Boden's three dimensions differentiable?} A one-way analysis of variance (ANOVA) carried out to evaluate the difference between the three score sets reveals a statistically significant difference between at least two groups (F(2) = 14.9, p $<$ 0.005). A Tukey’s HSD Test for multiple comparisons found that the mean of value scores (mean = 4.12) was significantly different than the means of novelty and surprise scores (mean = 3.72, p = 0.001, and mean = 3.86 p = 0.0018, respectively). However, there was no statistically significant difference between the means of novelty and surprise scores (p = 0.119) (see Figure \ref{fig:dist_scores}).

\textbf{Does musical training have an effect on creativity scores}. Subjects were segmented in three levels –low, mid, and high– according to their reported musical training to observe if the musical training has a significant effect on the three creativity scores. 

A one-way ANOVA shows that highly trained subjects gave significant different scores to at least two groups
(F(2) = 7.25, p = 0.0007) (see Figure \ref{fig:training_effect}). A subsequent Post Hoc Tukey test for multiple comparisons found that the differences between the scores of the value-novelty pair (mean 4.24, sd= 1.68 and mean = 3.61, sd=1.63, respectively) as well as the value-surprise ones (surprise mean =3.76, sd=1.62) were statistically significant (p = 0.00083 and p = 0.01663 respectively), but not for the novelty-surprise pair (p = 0.64244) (see Table \ref{tab:attribute_pair_training_level}).

There was also a statistically significant difference for at least two groups of scores of subjects with mid musical training (F(2) = 5.756, p = 0.0033). The Post Hoc Tukey HSD tests show that the scores of the value-novelty pair (mean=4.34, sd=1.23 and mean=3.99, sd=1.07, p = 0.00243, respectively) are significantly different (p = 0.00243), while the ones of the value-surprise (mean=4.11, sd=1.07) and novelty-surprise pairs are not (p = 0.08534, p = 0.43779 respectively). Finally, there was a statistically significant difference for the scores of at least two groups of subjects with low musical training level (F(2) = 3.4857, p = 0.031). The Post Hoc Tukey HSD tests show that value-novelty scores (mean=3.87, sd=1.44 and mean=3.56, sd=1.44 respectively)  have a significant difference (p = 0.0229137), and no significant difference between value-surprise (mean=3.73, sd=1.46) or novelty-surprise scores (p = 0.4016408, p = 0.3700743 respectively). 

For highly musically trained subjects, value scores are significantly different from novelty and surprise scores but novelty and surprise scores are indistinguishable from each other. Ratings of novelty surprise and value for all pieces by highly trained subjects have higher standard deviations (1.68, 1.63, 1.62) than those of low trained subjects (1.44, 1.46, 1.44), and those of mid trained subjects (1.07, 1.07, 1.23). Echoing \cite{maguire2011making}, results reveal that a highly surprising artifact for an expert might pass as routinary to a novice.
 


%For subjects with high musical training value scores are significantly different from novelty and surprise scores but novelty and surprise scores are indistinguishable from each other.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% table generated with https://www.tablesgenerator.com/latex_tables

\begin{table*}
\caption{Tukey HSD Post Hoc tests of significance for the difference between attribute ratings for three music training levels (low, mid, and high). Significant values marked with *}
\label{tab:attribute_pair_training_level}

\begin{tabular}{llll}
\hline
                   & \multicolumn{3}{c}{Attribute pair}                                                                            \\ \cline{2-4} 
Training & \multicolumn{1}{c}{value-novelty} & \multicolumn{1}{c}{value-surprise} & \multicolumn{1}{c}{novelty-surprise} \\ \hline
high               & 0.00083*                          & 0.01663*                           & 0.64244                              \\
mid                & 0.00243*                          & 0.08534                            & 0.43779                              \\
low                & 0.0229137*                        & 0.4016408                          & 0.3700743                           
\end{tabular}%
\end{table*}

\textbf{Are creativity scores similar across training groups?} A complementary analysis was carried out having musical training as treatments and creativity attributes as categories (see Figure \ref{fig:training_effect} and Table \ref{tab:training_level_attribute_score}). This serves to identify similarities between subject's assessment of pairs of creativity attributes. 

A one-way ANOVA revealed that there was a statistically significant difference in novelty scores between at least two groups (F(2) = 5.38, p = 0.0048). Tukey’s HSD Test for multiple comparisons found that novelty scores were significantly different between high and mid musical training (p = 0.04) and between mid and low musical training (p = 0.004). There was no statistically significant difference for novelty scores between high and low musical training (p = 0.899). A one-way ANOVA revealed that there was a statistically significant difference in surprise score between at least two groups (F(2) = 4.95, p = 0.0073). Tukey’s HSD Test for multiple comparisons found that the surprise scores were significantly different between mid and low musical training (p = 0.005) . There was no statistically significant difference between high and mid musical training (p = 0.101) and between high and low music training (p = 0.722). A one-way ANOVA revealed that there was a statistically significant difference in value scores between at least two groups (F(2) = 7.30 p = 0.0007). Tukey’s HSD Test for multiple comparisons found that value scores were significantly different between high and low musical training (p = 0.0198) and between mid and low musical training (p = 0.0011). There was no statistically significant difference between high and mid musical training (p = 0.789). Mid and low trained subjects’ scores are significantly different for all attributes, high and low trained subjects have significantly different value scores, while high and mid trained groups have significantly different novelty scores. The scoring ranges of novelty and surprise are very similar among them for all subject segments but value score’s standard deviation is higher than that of novelty and surprise scores in high and mid trained subjects (1.679 vs 1.608, 1.607 and 1.242 vs 1.092, 1.081 respectively) but not in low-trained subjects in which the opposite effects is observed: value scores are less disperse than those of novelty and surprise (1.406 vs 1.449, 1.460). 


\begin{figure*}[ht]
\centering
\includegraphics[width=1\textwidth]{training_effect.png}
\caption{Novelty, surprise and value at three different musical training levels: high, mid and low (left, bottom, right respectively)}
\label{fig:training_effect}
\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% table generated with https://www.tablesgenerator.com/latex_tables
\begin{table*}[]
\caption{Tukey HSD post hoc tests of significance for the difference between high, mid, and low levels of musical training.  Significant differences marked with *}
\label{tab:training_level_attribute_score}
\begin{tabular}{lccc}
\hline
          & \multicolumn{3}{c}{Training level} \\ \cline{2-4} 
Attribute & High-Mid   & High-Low   & Mid-Low  \\ \hline
Novelty   & 0.04*      & 0.89       & 0.004*   \\
Surprise  & 0.101      & 0.722      & 0.005*   \\
Value     & 0.789      & 0.019*     & 0.001*  
\end{tabular}%
\end{table*}


%To further investigate the effect of training on the creativity attribute’s scores, subjects were segmented by their reported musical training scores in two groups: low musical training (1, 2, 3) and high musical training (4, 5, 6) (See Figure \ref{fig:traininhg_effect2}). Three two-sample t-tests were performed to compare novelty, surprise and value in the group with low training and high training. The result shows no significant difference in novelty scores between high musical training (M = 3.677, SD = 1.456) and low musical training (M = 3.73, SD = 1.37); t(df) = -0.546, p = 0.584. There was no significant difference in surprise scores between high musical training (M = 3.829, SD = 1.46) and low musical training (mean = 3.882, SD = 1.366); t(df) = -0.478, p = 0.316. Finally, there was a significant difference in value scores between high musical training (mean = 4.262, SD = 1.542) and low musical training (mean = 4.03, SD = 1.372); t(df) = 2.033, p = 0.042. 

The effect of training in value scores has proven to be statistically significant between mid and low training. The analysis reveals that the standard deviation of highly trained subjects’ scores is significantly greater than the ones of the rest of the subjects.  

\begin{figure*}[ht]
\centering
\includegraphics[width=1\textwidth]{training_effect2.png}
\caption{Novelty, surprise and value at two different musical training levels: high (left) and low (right)}
\label{fig:traininhg_effect2}
\end{figure*}


%% THIS SECTION IS ABOUT TIMBER ASSISTANT. IT IS COMMENTED BY THE \iffalse ... \if SECTION.

\iffalse
\textbf{The effect of using a timbre assistant}. A Welch t-test was performed to evaluate to what extent the subject's assessment of stimuli was affected by the two timbre conditions: timbre assistant system and static timbre setting. The results show statistically significant differences between the respective means of novelty, value, and surprise scores of both treatments (See Table \ref{tab:training_level}). Overall, the distribution of scores of both treatments (presented in Figure \ref{fig:dist_novelty}) shows a similar negative skewness, but different kurtosis. While the distribution of timbre assistant scores are leptokurtic and divergent, the static timbre setting scores are mesokurtic and homogeneous. Value has the highest frequency of responses followed by surprise and novelty in both conditions.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% table generated with https://www.tablesgenerator.com/latex_tables
\begin{table*}
\caption{Welch t-tests comparing the scores of the three attributes for pieces created with and without the timbre assistant}
\label{tab:training_level}
\begin{tabular}{lcccccc}
\hline
          & \multicolumn{2}{c}{Timbre assistant system} & \multicolumn{2}{l}{Static timbre setting} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5}
Attribute & mean                  & SD                  & mean                & SD                  & t                    & p-value              \\ \hline
Novelty   & 4.025                 & 1.46                & 3.57                & 1.36                & t(452)=4.07          & \textless{}0.05      \\
Surprise  & 4.2                   & 1.41                & 3.69                & 1.37                & t(460)=4.67          & \textless{}0.05      \\
Value     & 4.33                  & 1.48                & 3.98                & 1.41                & t(460)=3.05          & \textless{}0.05     
\end{tabular}%

\end{table*}

\begin{figure*}
\centering
\includegraphics[width=1\textwidth]{dist_novelty.png}
\caption{Distribution of novelty, surprise and value scores for stimuli created with a static timbre setting (left) and the timbre assistant system (right)}
\label{fig:dist_novelty}
\end{figure*}

Overall, the stimuli generated with the timbre assistant are perceived as more valuable, surprising and novel. An analysis of the aggregated mode of scores (equivalent to a creativity score) for each stimulus presented in Figure \ref{fig:dist_scores} shows that most of the stimuli generated with the timbre assistant (pieces 11, 9, 13, 2, 18 and 15) score above the creativity score mean (12.16), whereas most of the ones generated with the static timbre setting scored below the mean. The aggregated mode is equivalent to a creativity score. Stimulus 11 unanimously scored the maximum mode in all three attributes. 

\begin{figure*}[ht]
\centering
\includegraphics[width=1\textwidth]{sorted_creativity_score.pdf}
\caption{Stimuli sorted by creativity score and differentiated by timbre assistance. The  creativity score is the aggregated of novelty, surprise, and value}
\label{fig:creativity_score}
\end{figure*}
\fi
